Unsupervised Out-of-Domain Detection via Pre-trained Transformers

Deployed real-world machine learning applications are often subject to uncontrolled and even potentially malicious inputs. Those out-of-domain inputs can lead to unpredictable outputs and sometimes catastrophic safety issues. Prior studies on out-of-domain detection require in-domain task labels and are limited to supervised classification scenarios. Our work tackles the problem of detecting out-of-domain samples with only unsupervised in-domain data. We utilize the latent representations of pre-trained transformers and propose a simple yet effective method to transform features across all layers to construct out-of-domain detectors efficiently. Two domain-specific fine-tuning approaches are further proposed to boost detection accuracy. Our empirical evaluations of related methods on two datasets validate that our method greatly improves out-of-domain detection ability in a more general scenario.

==> backup/conclusion.tex <==

\vspace{-.2em}
\section{Related Work} 
\vspace{-.5em}
Two lines of works are proposed to perform out-of-domain detection. 
One is to tackle the problem in specific classification tasks, where well-trained classifiers are utilized to design anomaly scores \citep[e.g.,][]{hendrycks2016baseline,liang2018enhancing,lee2018simple,hendrycks2020pretrained}, which limits their application scenarios.
Another line of work is based on support estimation or density estimation, which assumes the in-domain data is in specific support or from the high density region \citep{scholkopf2001estimating,tax2004support}. \citet{pmlr-v48-zhai16,ruff2018deep} also leverage the features of neural networks, though requiring to design specific network structures for various data.
In this work, we avoid the issues of prior works by designing a computationally efficient method utilizing the representations of pre-trained transformers.
\vspace{-1em}
\section{Conclusion}
\vspace{-.3em}
We study the problem of detecting out-of-domain samples with unsupervised in-domain data and believe this is a more general setting for out-of-domain detection. We propose a simple yet effective method which significantly improves the detection ability.
Two domain-specific fine-tuning techniques are further explored to boost the detection performance.





==> backup/experiments.tex <==


\begin{table*}[t]
 \setlength{\tabcolsep}{8pt}
		\renewcommand{\arraystretch}{1.02}
		\centering
\scalebox{.91}{
\begin{tabular}{l|cccc|cccc}
\toprule
 & \multicolumn{4}{c}{SST} & \multicolumn{4}{c}{CLINIC150} \\ 
  & \multicolumn{8}{c}{~~~AUROC $\uparrow$~~ / ~~DTACC $\uparrow$~~ /~~ AUIN $\uparrow$~~ / ~~AUOUT $\uparrow$~~} \\ \midrule\midrule
BERT-single layer $\dagger$                   & 82.9  & 74.8  & 81.3 & 84.4  & 64.6 & 60.9 & 88.4 & 26.7  \\
BERT-single layer + BCAD $\dagger$                   &  91.7 & 87.9 & 93.5 & 87.7 & 70.8 & 65.61 & 89.1 & 43.1 \\
BERT +  Ours  $\dagger$                &  97.5  &  89.9 & 97.9 & 97.1 & 76.7 & 71.1 &  93.4 & 38.2 \\
BERT + IMLM +  Ours  $\dagger$           & 97.4  &   92.7 & 97.8 & 97.0 & 77.7 & 72.1 & 93.8 & 39.0    \\
BERT + BCAD +  Ours $\dagger$       & 96.2 & 91.7 & 97.1 & 94.3 & $\textbf{82.2}$ &  $\textbf{74.5}$ &  $\textbf{95.0}$ & $\textbf{53.0}$   \\
\midrule\midrule
RoBERTa-single layer  $\dagger$              &  72.7   &  82.0 & 58.1 & 84.0 & 59.9 & 57.5 & 86.7 & 22.6 \\
RoBERTa-single layer + BCAD  $\dagger$              &  99.7 &  99.0 &  99.6 &  99.6  &  65.8 & 62.1 & 87.8 & 37.4 \\
RoBERTa +  Ours   $\dagger$      & 99.8  & 97.7 & 99.8  & 99.8 & 78.6 & 71.9 & 93.8 & 42.6  \\
RoBERTa + IMLM +  Ours $\dagger$   &  $\textbf{99.9}$  & 97.7 & $\textbf{99.8}$ & $\textbf{99.8}$  & 80.1 & 73.1 & 94.5  & 44.9      \\
RoBERTa + BCAD +  Ours $\dagger$   & 99.2 & 98.7 & 99.5  & 98.5  & 79.8 & 72.6 & 94.1 & 49.3   \\
\midrule\midrule
TF-IDF $\dagger$                  &   61.1 &  63.2 & 52.5   & 63.5   & 60.8  &  58.8  &  85.6    &24.3 \\
BERT +BCAD + MSP             & 83.6 & 74.5 & 83.8 & 83.5 & 71.3	& 65.8&	90.0&	43.6 \\
RoBERTa + BCAD + MSP           &  99.2  & \textbf{99.2} & 99.5 & 98.0 & 66.0  &  62.0  &  88.7  & 31.6    \\
\bottomrule
\end{tabular}
}
\vspace{-.3em} 
\caption{\small{Results on SST and CLINIC 150. For SST dataset, out-of-domain samples are from the other four datasets. For CLINIC 150,  out-of-domain samples are manually labeled.  $\dagger$ indicates that OC-SVM are used for computing anomaly scores, once the feature is extracted. Best results are marked in bold.} }
\label{tab:results}
 \vspace{-0.5em}
\end{table*}

\vspace{-.1em}
\section{Experiments}
\label{sec:exp}
\vspace{-.7em}
\paragraph{Datasets}
We use two different datasets for evaluation, where one is for detecting out-of-domain text from unseen datasets, and the other one for detecting class-level out-of-domain sentences from the same dataset.

$\bullet$ \textbf{SST}: We follow the experimental settings in~\citet{hendrycks2020pretrained}, by providing the training samples from the SST dataset~\citep{Socher2013RecursiveDM}, 
and consider the samples from the other four datasets as out-of-domain data, including 20 Newsgroups~\citep{Lang1995NewsWeederLT}, English-German Multi30K~\citep{Elliott2016Multi30KME}, RTE~\cite{Dagan2005ThePR} and SNLI~\citep{Bowman2015ALA}.
For evaluation, we use the test data of SST as in-domain positives, and randomly pick 2000 samples from the four datasets as out-of-domain negatives. 
Note that we do not use the labels of all samples.

$\bullet$ \textbf{CLINIC150}: CLINIC150 \citep{larson2019eval} is a new crowdsourced dataset, including in-domain queries covering 150 intents, and out-of-domain queries, which do not fall within any of the 150 intents.
We use all 15,000 training sentences, and mix the 4,500 testing samples with 1,000 out-of-domain sentences for evaluation.
This is  a more challenging task since the out-of-domain samples are collected by human labors. Illustrative sentences of the dataset can be found in Table \ref{tab:example_sentences}.

\vspace{\vspa}
\noindent\textbf{Evaluation Metrics}~~~~
We follow \citet{liang2018enhancing} to report four different metrics, including Detection Accuracy (\textbf{DTACC}), Area Under the Receiver Operating Characteristic Curve (\textbf{AUROC}) and Area under the Precision-Recall curve (\textbf{AUPR}) for in-domain and out-of-domain testing sentences respectively, denoted by AUIN and AUOUT. 

\vspace{\vspa}
\noindent\textbf{Model Configurations}~~~~
We evaluate all methods with both BERT and RoBERTa (\texttt{base} models with 768 latent dimensions).
For BCAD fine-tuning, we consider CLINIC150 as the auxiliary dataset for SST, and vs versa. Notice that the test data \textit{does not contain} any samples from the auxiliary dataset.

\vspace{\vspa}
\noindent\textbf{Choice of $f_{\ell}$}~~~~
We evaluate both [CLS] token and averaging contextualized vectors of each tokens at the $\ell$-th layer of the model $f$, and report the best results for all methods.

\vspace{\vspa}
\noindent\textbf{Baselines}~~~~ 
To examine the effectiveness of our newly proposed anomaly scores that can utilize the representations of all layers, we compare it with the following three baselines:

    $\bullet$ (Ro)BERT(a)-single layer: we consider the representation $f_{\ell}$ as the OC-SVM input.
    We iterate all 12 layers and report the best results. 
    Details of probing results of each layer in Table \ref{tab:results-cls} and Table \ref{tab:results-average} in the Appendix. 
    
    $\bullet$  TF-IDF: We extract frequency-based features as the input of OC-SVM. We use SVD to convert high-dimensional features to 100-dimension for computational efficiency. 
    
    $\bullet$  BCAD + MSP: We test maximum of softmax probability (MSP), which is considered in prior works \citep{liang2018enhancing,hendrycks2020pretrained}. 
    Notice that we can only test MSP using the transfomers fine-tuned by BCAD.





\vspace{\vspa}
\noindent\textbf{Results}~~~~ 
We report evaluation results in Table~\ref{tab:results}.
As we observe that detecting out-of-domain samples for CLINIC150 is more challenging than that of cross-dataset out-of-domain data in SST, this is mainly because the out-of-domain samples in CLINIC150 are annotated by humans and are closer to the in-domain samples in language.

Methods with single-layer feature $f_{\ell}$ from pre-trained transformers also achieve better performance, compared with the method based on features extracted by TF-IDF. 
Though our method requires more assumptions on the features, it significantly outperforms other baselines. 
Notice that our approach is also more computationally efficient when obtaining optimal $\pmb{w}$ and $\pmb{R}$ since the optimization is performed on a new transformed low dimensional data space ($d = 12$).


Both of our designed domain-specific fine-tuning, IMLM and BCAD, can further boost detection performance. 
In CLINIC150, the improvements introduced by using BCAD are significant. 
The best results are achieved by BERT + BCAD + Ours. 
MSP, which can only be calculated on the models finetuned by BCAD, performs well for detecting cross-dataset outliers, while the performance drops significantly when evaluated on the challenging CLINIC150 dataset.

Besides, we observe that methods based on BERT are better at handling realistic out-of-domain samples (CLINIC150), and the methods based on RoBERTa outperform BERT-based ones at identifying samples from the other datasets. 
%The results are pretty consistent when combined with different fine-tuning methods. 


\vspace{\vspa}
\noindent\textbf{Visualizations}~~~~ 
Figure~\ref{fig:aurocs} (a) plots the ROC curves of three different anomaly scores on CLINIC150, validating our method has significantly better detecting ability compared with the other two baselines. 
We also report the distribution of anomaly scores generated by our method in Figure~\ref{fig:aurocs}~(b).






\newcommand{\gapp}{-1.5em}

\begin{figure}[t]
    \centering
     \begin{tabular}{cc}
        \includegraphics[height=0.40\linewidth]{Figures/auroc-3.pdf} &
        \hspace{\gapp}
         \includegraphics[height=0.40\linewidth]{Figures/hist.pdf}
         \vspace{-.2em}\\
        
        \footnotesize{(a)  ROC Curves} &\hspace{\gapp} \footnotesize{(b) Anomaly score distribution} \\
    \end{tabular}
    \vspace{-1em}
    \caption{\small{(a): ROC Curves of three anomaly scores on CLINIC150. (b): Distribution of anomaly scores generated by BCAD + Ours. Both figures are based on the BERT model.}}
    \label{fig:aurocs}
    \vspace{-1em}

\end{figure}

==> backup/intro_back.tex <==
\section{Introduction}
Deep neural networks, despite achieving good performance on many challenging tasks, can make high confidence predictions for completely irrelevant, out-of-domain inputs, leading to significant AI safety issues~\cite{hendrycks2016baseline}. 
Detecting out-of-domain inputs is a fundamental task for trustworthy AI applications in real world use cases, because those applications are often subject to ill-defined queries or even potentially malicious inputs. 
%Out-of-domain detection is a necessary building block for trustworthy application of machine learning models, due to the potential misspecified or even malicious examples that the model can encounter in real world scenarios.
%Prior works \citep[e.g.,][]{hendrycks2016baseline,lee2018simple,liang2018enhancing,hendrycks2018deep,hendrycks2020pretrained} have considered out-of-domain detection with well-trained multi-class classifers, which require labels and also limit the task domain to multi-class classifications.
Prior work on out-of-domain detection \citep[e.g.,][]{hendrycks2016baseline,lee2018simple,liang2018enhancing,hendrycks2018deep,hendrycks2020pretrained} mostly required labels, limiting its usage to classifications tasks.
%These requirements can highly constrain their applications in real-world scenarios, where the tasks depend on unlabeled data from internet (\textcolor{red}{(ADD citation) e.g., wiki, common crawl dataset}).
% On the other hand, the out-of-domain detection problem itself does not require well-trained classifiers or labels.
However, deployed applications rarely receive controlled inputs, and are susceptible to an ever-evolving set of user inputs that are scarcely labeled. 
Therefore, it is natural to ask the following question:

\emph{Can we detect out-of-domain samples using only in-domain data without labels?}

%Notice that, out-of-domain detection itself is equivalent to check whether the given test samples are drawn from the same distribution that generates the in-domain samples.The equivalent problem we study here requires the weakest assumption than prior works \citep{hendrycks2020pretrained}, that only assumes we have the in-domain samples, which further allows us to understand the statistical properties of data itself regardless of the tasks, which makes the methods developed for this problem more applicable than the task specific out-of-domain detection methods\citep[e.g.,][]{lee2018simple,hendrycks2020pretrained}.

%Notice that this problem assume the \emph{weakest} condition for out-of-scope detection, i.e. the access to the data distribution or the dataset, without \emph{any} assumption on the availability of the additional information, e.g. the label information. And in most of the case, we should have the dataset to train the machine learning models, and thus the assumption should be simply satisfied. Also, understanding out-of-scope detection as the property testing can get rid of the dependency on the task, as the only thing we need is the data distribution or the dataset, and thus the property testing based methods can be more flexible than the task-specific out-of-scope detection methods. {\color{red} have a better description other than property testing?}
We regard the out-of-domain detection problem as checking whether the given test samples are drawn from the same distribution that generates the in-domain samples, which requires the weakest assumption among prior works \citep[e.g.,][]{lee2018simple, hendrycks2020pretrained}.
We suppose that we only have in-domain samples, which allows us to understand the properties of data itself regardless of tasks; therefore, the methods developed for this problem are more applicable than task specific ones, and can be further adapted to tasks where no labels were present, such as active learning or transfer learning.



To solve the problem, 
we utilize the latent embeddings of pre-trained transformers \citep[e.g.,][]{vaswani2017attention,devlin-etal-2019-bert,liu2019roberta} to represent the raw data, which allows us to apply classical out-of-domain detection methods such as one class support machines \citep{scholkopf2001estimating}  or support vector data description \citep{tax2004support} on the latent representations of the pre-trained transformers.
Besides, we also develop a simple yet effective out-of-domain detection method that is computationally efficient and utilizes the representations of all layers, which significantly improves the ability of detecting outliers compared with methods that can only use representations of the one or two layers.

%\paragraph{Outlines} \textcolor{red}{may remove}
%In Section \ref{sec:setup} we formally introduce the problem of out-of-domain detection and the general idea of constructing outlier detectors.
%Section ~\ref{sec:pretraining_models} describes three different strategies to obtain or improve the representations of pre-trained transformers.
%Based on the models and representations obtained from %Section~\ref{sec:anomal_scores}, we discuss possible anomaly detectors, and also propose a simple method that can utilize the latent embeddings of all layers. 
%Finally, in Section \ref{sec:exp} we evaluate all methods discussed in this paper and conclude that our proposed outlier detection strategy can achieve significantly better outlier detecting performance using the latent representations of pre-trained transformers.







==> backup/method.tex <==

\section{Problem Setup}

\label{sec:setup}
%In this paper, we consider the problem of anomaly detection without labels.
Assume that we have a collection of text inputs $\mathcal{D}_{n} := \{\pmb{x}_i\}_{i=1}^{n}$ \textbf{without any in-domain labels};
we want to construct an out-of-domain detector that can output an anomaly score when given a new input $\pmb{x}$. This detector can determine whether $\pmb{x}$ comes from the same distribution that generates $\mathcal{D}_{n}$, and it
can be described mathematically as:
$$
    g(\pmb{x}, \epsilon) = \begin{cases}\rm{\textbf{True}} & \rm{if} ~~\mathcal{I}(\pmb{x}) \leq  \epsilon\,, \\ \rm{\textbf{False}} & \rm{if} ~~\mathcal{I}(\pmb{x}) > \epsilon\,, \end{cases}
$$
where $\mathcal{I}(\pmb{x})$ is the anomaly score, and $\epsilon$ is a chosen threshold to ensure that the true positive rate is at certain rate (e.g. $95\%$) ~\citep{hendrycks2016baseline,liang2018enhancing,lee2018simple}. 
% \keyang{just say a certain rate instead of using a specific number?}
The outlier detection problem boils down to designing the anomaly score $\mathcal{I}(\pmb{x})$. 
%So the key step for constructing outlier detectors is to design the anomaly score $\mathcal{I}(\pmb{x})$.
Besides, we assume that we \textbf{have no prior knowledge} of out-of-domain samples when constructing $\mathcal{I}$.

Without access to labels, it is natural to resort to classic outlier detection methods like one-class support vector machine \citep{scholkopf2001estimating}, support vector data description \citep{tax2004support} or kernel density estimation (KDE) for estimating the support or the density of the in-domain data distribution.
%When we do not have access to the labels, an immediate solution is to utilize existing pure sample based outlier detection methods. Classic methods include one-class support vector machine \citep{scholkopf2001estimating}, support vector data description \citep{tax2004support} or kernel density estimation (KDE) for estimating the support or the density of the in-domain data distribution.
%However, kernel based methods often fail in high dimensional scenarios and it is also difficult to design kernels for different types of sentences.
However, such methods often fail in high dimensional scenarios, and handcrafting representations for different types of sentences can be laborious. In this paper, we propose to construct out-of-domain detectors with unlabeled data from the representations of large scale pre-trained models \citep[e.g.,][]{devlin-etal-2019-bert,liu2019roberta}, and investigate how to efficiently and effectively leverage these representations.
%Instead of constructing detectors on raw sentences $\{x_i\}_{i=1}^{n}$, we propose to obtain outlier detectors on the representations of large scale pre-trained models \citep[e.g.,][]{devlin-etal-2019-bert,liu2019roberta}.
Specifically, we aim to address the two problems below in the following sections:

    $\bullet$ What kind of representations or models can be utilized to distinguish in-domain and out-of-domain sequences?
    
    $\bullet$ Based on the representations presented, how can we design anomaly scores to discover new out-of-domain sequences?

\section{Model and Feature Learning}
\label{sec:pretraining_models}

We utilize features obtained from pretrained transformers such as BERT \citep{devlin-etal-2019-bert} or RoBERTa \citep{liu2019roberta} for constructing outlier detectors in lieu of labels for samples in $\mathcal{D}_{n}$. Moreover, we explore two fine-tuning techniques. 
%Since we do not have labels for sentences in $\mathcal{D}_{n}$, we can utilize features of pretrained transformers such as BERT \citep{devlin-etal-2019-bert} or RoBERTa \citep{liu2019roberta} for constructing outlier detectors.
%Besides, we also study two possible fine-tuning techniques that may be helpful for the latter outlier detectors, which we describe below.

\paragraph{In-domain Mask Language Modeling (IMLM)}
Besides directly using pretrained features of BERT, we also fine-tune the model on the training dataset $\mathcal{D}_{n}$ using mask language modeling~ \citep{devlin-etal-2019-bert}. 
%The intuition is that by fine-tuning the model on the training data, the features might concentrate, allowing us to study the properties of the training features to find outlier samples.
The reason why we further fine-tune the model on the training data is that we hope the features of the training data will concentrate,
allowing us to study the properties of the training features to find outlier samples.

\paragraph{Binary Classification with Auxiliary Dataset (BCAD)}
Another way we fine-tune the pretrained transformers is to introduce an auxiliary dataset and perform a binary classification task. We consider the training data in $\mathcal{D}_{n}$ as positive samples and data in the auxiliary dataset as negative samples. 
%We can also introduce another dataset, which does not need to be part of the OOD data at test time.  Consider the training data in $\mathcal{D}_{n}$ as positive samples and auxiliary dataset as negative samples, then we can fine-tune the model with a binary classification task.
After training, we can either use the maximum of softmax prediction (MSP) of the binary classifier as the anomaly score \citep{hendrycks2016baseline,hendrycks2018deep,hendrycks2020pretrained}, or use the representations of the models to construct anomaly scores, which we describe in Section~\ref{sec:anomal_scores}. 
Notice that obtaining such datasets can be easy since we can use all available public datasets, and there are no limitations on the auxiliary datasets.




\section{Anomaly Scores $\mathcal{I}(\pmb{x})$}
\label{sec:anomal_scores}
Suppose we have a model $f(\pmb{x})$ obtained from Section \ref{sec:pretraining_models}, and our next step is to use $f(\pmb{x})$ to design anomaly scores $\mathcal{I}(\pmb{x})$ for detectors. In this section, we introduce three different out-of-domain detectors later studied in our empirical experiments.
For notation simplicity, we assume the model $f$ has $L$ layers, i.e. $f = f_{L}\circ f_{L-1} \circ \cdots \circ f_1$, where $\circ$ denotes the composition function, and $f_{\ell}$ is the embedding corresponding to the $\ell$-th layer.
We use $f_{\ell}(\pmb{x}):= f_{\ell} \circ \cdots\circ f_{1}(\pmb{x})$ for short.


\paragraph{Maximum Softmax Probability (MSP)} Suppose $f(\pmb{x})$ is trained with BCAD, then we can use maximum calibrated softmax probability with temperature scaling as the anomaly score \citep{liang2018enhancing,hinton2015distilling}:
$
    \mathcal{I}(\pmb{x}):= \max_{i \in \{1, 2\}} \frac{\exp\left(h_i(\pmb{x})/ T\right)}{\sum_{j=1}^{2}\exp\left(h_j(\pmb{x})/ T\right)}, 
$
 where $h_i(\pmb{x})$ is the output logits of the binary classifier, 
 and $T$ is the temperature that is selected such that the true positive rate is at a given rate ($95\%$ in \citet{liang2018enhancing}).
 

\paragraph{Outlier Detection with Embeddings from $\ell$-th Layer $f_{\ell}$}

We can utilize existing pure sample based methods, such as one-class support vector machine (OC-SVM) to construct detectors on features from the $\ell$-th layer $f_{\ell}$. For each input $\pmb{x_i}$, we can either use the embedding of [CLS] token, or the mean of contextualized embeddings of tokens at the $\ell$-layer to obtain a single vector. 
Then we can directly construct an outlier detector based on the transformed features of each sentences in $\mathcal{D}_{n}$ using OC-SVM.
% In our experiments, we  perform a probe study to understand the embeddings of which layer can improve the outlier detecting ability. By default, we use the last layer $f_{L}(\pmb{x})$ to construct outlier detectors. TODO check}

However, using the representations from one or two layers to construct effective anomaly scores might not suffice. Concatenating features of all layers might be computationally expensive for OC-SVM, and kernel based methods tend to fail in high dimensional scenarios. 
To tackle these problems, we propose a simple yet effective method (described below) that utilize latent representations of all layers and can automatically decide which layers are more important.

\paragraph{Outlier Detections with All Features of $f(\pmb{x})$}

% \paragraph{Incorporating Levels of Features}

% Given access to pre-trained models,
% a practical choice to utilize them is using the feature before the softmax layer as the feature of the data, i.e. $\Phi(\bm{x}) = f(\bm{x})$. 
% With this kind of feature, there exist several feature-based methods that we can directly apply, for example, 
% one-class classification based methods \cite{scholkopf2001estimating, tax2004support}.
% However, the output from different layers can provide different level of features. 
% For convolutional neural networks that are widely used in the image domain, the bottom layers focus more on the texture information, while the top layers focus more on the shape information.
% As a consequence, 
% we would like to utilize the features from different levels,
% so we consider the following feature instead of $f$:
% {
% \begin{align}
%     \Phi(\bm{x}) = [f_1(\bm{x}), f_2\circ f_1(\bm{x}), \cdots, f_L \circ \cdots \circ f_1(\bm{x})]\,.
%     \label{eq:feature}
% \end{align}}

% \paragraph{Ellipsoidal Data Description}

% Traditional one-class classification assumes the feature of the in-distribution data and the out-of-domain data can be separated by simple surfaces like hyper-plane (one-class SVM) and hyper-sphere (SVDD). 
% However, the feature provided by deep models may not be separable with such surfaces. 
% In this paper, we focus on a generalization of the hyper-sphere called hyper-ellipsoid, which can be defined by:
% {
% \begin{align}
%     \|\Phi(\bm{x}) - \bm{c} \|_{\bm{\Sigma}^{-1}}^2 = (\Phi(\bm{x}) - \bm{c})^\top \bm{\Sigma}^{-1} (\Phi(\bm{x}) - \bm{c}) = R^2\,,
% \end{align}}
% where $\Phi$ is the feature map, $\bm{c}$ is the center of the hyper-ellipsoid, $\bm{\Sigma}$ is a symmetric positive definite matrix, which reflects the shape of the ellipsoid.
% And $R$ reflects the volume of the hyper-ellipsoid.\footnote{We can further assume $\|\bm{\Sigma}\| =1$, where the norm can be operator norm, Frobenius norm or the operator norm, which can give the definition of the hyper-ellipsoid with unique $\bm{\Sigma}$ and $R$.}
% We consider the following optimization problem to find the hyper-ellipsoid:
% \begin{align}
%     &\min_{R, \bm{c}, \bm{\Sigma}, \bm{\xi}} \frac{1}{2}\|\bm{\Sigma}\|_{\text{Fr}}^2 + \left(R^2 + \frac{1}{\nu n}\sum_i \xi_i\right)\,, \notag \\
%     &\quad \text{s.t.}\quad \|\Phi(\bm{x}_i) - \bm{c}\|_{\bm{\Sigma}^{-1}}^2 \leq R^2 + \xi_i\,, \quad \xi_i \geq 0\,,\forall i\,.
%     \label{eq:objective}
% \end{align}
% Here we introduce a regularization term $\frac{1}{2} \|\bm{\Sigma}\|_{\text{Fr}}^2$ to constrain the complexity of $\bm{\Sigma}$. If $\bm{\Sigma} = \bm{\mathrm{I}}$, then the optimization problem is identical to one-class SVDD. After we find the optimal $R$, $\bm{c}$ and $\bm{\Sigma}$, we can view a new sample $\bm{y}$ as out-of-domain data, if $\Phi(\bm{y})$ isn't in the hyper-ellipsoid  $\|\Phi(\bm{x}) -\bm{c}\|_{\bm{\Sigma}^{-1}}^2 = R^2$.


% \paragraph{A Practical Approximation for Solution}\quad\quad
% To solve Problem \eqref{eq:objective} exactly can be painful, since solving Problem \eqref{eq:objective} involves finding the optimal $\bm{\Sigma}$ of shape $d \times d$, where $d$ is the dimension of the feature. 
% For the features we defined in Eq. \eqref{eq:feature}, 
% $d$ can be tens of thousands or even hundreds of thousands, 
% which makes the exact solution equipped with the features in Eq. \eqref{eq:feature} computational intractable.
% We instead propose a \textbf{simple and computationally efficient} approximation for the solution that can be useful in practice.

% First, we decompose the feature space into several subspace,
% based on the feature from different layers, i.e. assume $\bm{\Sigma}$ is a block diagonal matrix:
% \begin{align*}
%     \bm{\Sigma}=\left[
% \begin{array}{ccccc}
% \bm{\Sigma}_1& & & & \\
% &\bm{\Sigma}_2& & & \\
% & & &\ddots&  \\
% & & & &\bm{\Sigma}_L\\
% \end{array}\right]\,,
% \end{align*}
% where $\bm{\Sigma}_\ell$ reflects the shape of feature distribution at layer $\ell$. And with a straightforward calculation, we have:
% \begin{align*}
%     \|\Phi(\bm{x}) - \bm{c}\|_{\hat{\bm{\Sigma}}^{-1}}^2 = \sum_{\ell=1}^L \|f_{\ell}\circ f_{\ell-1}\circ\cdots \circ f_{1}(\bm{x}) - \bm{c}_\ell\|_{\bm{\Sigma}_\ell^{-1}}^2 \,.
% \end{align*}

We first calculate the Mahalanobis distance of the feature from test data for each layer, which can be written as $
M_\ell(\bm{x}) =  \|f_\ell(\bm{x}) - \hat{\bm{c}}_l\|^2_{\hat{\bm{\Sigma}}_l^{-1}}
$, where $\bm{c}_{\ell}$ and $\bm{\Sigma}_{\ell}$ are the empirical mean and the empirical covariance of the features from layer $\ell$ for in-domain data.
% We first calculate a score from the features from each layer. 
% For each layer $\ell$, we define the empirical mean $\hat{c}_\ell$ and empirical covariance $\hat{\Sigma}_\ell$ from the training data $\{\pmb{x}_i\}_{i=1}^n$:
% $\hat{\bm{c}}_\ell =  \frac{1}{n} \sum_{i=1}^n \left[ f_{\ell}(\bm{x}_i) \right]$,
% $\hat{\bm{\Sigma}}_\ell =  \frac{1}{(n-1)} \sum_{i=1}^n (f_{\ell}(\bm{x}_i) - \hat{\bm{c}}_\ell) (f_{\ell}(\bm{x}_i) - \hat{\bm{c}}_\ell)^\top\,.$
% Then we define the following score of data $\bm{x_i}$ at layer $\ell$ as:
% $
% M_\ell(\bm{x}_i) =  (f_{\ell}(\bm{x}_i) - \hat{\bm{c}}_\ell)^\top \hat{\bm{\Sigma}}_l^{-1}( f_{\ell}(\bm{x}_i) - \hat{\bm{c}}_\ell).
% $
% Intuitively, this score measures how the features of data $\bm{x}_i$ at the $\ell$-th layer deviate from $\hat{\bm{c}}_l$, the center of the feature from the training data, weighted by $\hat{\bm{\Sigma}}_l$, the shape of the feature from the training data. If $\bm{x}_i$ is generated from the data distribution, then each of $M_\ell(\bm{x}_i)$ should be small. 
Then, to measure the importance of the feature from each layer, we can use the one-class SVM,
% \keyang{we mentioned OC-SVM earlier, should we move the definition forward?}, 
whose formulation with linear kernel can be described as:
\begin{align*}
    & \min_{R, \bm{w}, \bm{\xi}} -\frac{1}{2}\|\bm{w}\|_2^2 + R^2 + \frac{1}{\nu n} \sum_i \xi_i\,, \notag\\
    & \quad \text{s.t.}\quad \langle \bm{w}, M(\bm{x}_i) \rangle \leq R^2 + \xi_i, \xi_i \geq 0\,, \forall i\,, \label{equ:our_obj}
\end{align*}
where $M(\bm{x}_{i}) = [M_{1}(\bm{x}_{i}), \ldots, M_{L}(\bm{x}_{i})]^{\top}$.
Here $\bm{w}$ measures the importance of the score from layer $\ell$, $R$ determines the decision boundary and $\xi_i$ is the slack variable used for a soft margin.
After we find the optimal $R$ and $\bm{w}$, for a new sample $\bm{u}$, we can calculate the anomaly score as 
$\mathcal{I}(\bm{x}) = \langle \bm{w}, M(\bm{x})\rangle - R^2$.

%{\color{red} In practice, we can also use one-class SVM with different kernels (e.g., polynomial kernel), which can measure the importance of the score from each layer in a more implicit way. }
%\keyang{I cannot sense the importance of using all features after reading the definition of OC-SVM. }

% \noindent\paragraph{The choice of the norm $\|\cdot\|_{\mathcal{F}}$}
% Note that, if we don't further fine-tune the pre-trained model, the features in the feature space is probably not enclosed by a hyper-sphere. Thus, use the Euclidean distance (i.e. the $\ell_2$ distance) like \citep{ruff2018deep} can be problematic. We focus on one generalization of hyper-sphere, namely hyper-ellipsoid. The hyper-ellipsoid can be defined by:
% \begin{align}
%     \|\Phi(\bm{x}) - c \|_{\Sigma^{-1}}^2 = (\Phi(\bm{x}) - c)^\top \Sigma^{-1} (\Phi(\bm{x}) - c) = R^2
% \end{align}
% where $c$ is the center of the hyper-ellipsoid, $\Sigma$ is a symmetric positive definite matrix reflects the shape of the ellipsoid\footnote{We can further assume $\|\Sigma\| =1$ where the norm can be operator norm, Frobenius norm or the operator norm, which can give the definition of the hyper-ellipsoid with unique $\Sigma$ and $R$.} and $R$ reflects the volume of the hyper-ellipsoid. We consider the following optimization problem instead of Eq. \eqref{eq:objective_svdd}:
% \begin{align}
%     \min_{R, c, \Sigma, \bm{\xi}} \frac{1}{2}\|\Sigma\|_{\text{Fr}}^2 + \left(R^2 + \frac{1}{\nu n}\sum_i \xi_i\right), \quad \text{s.t.}\quad \|\Phi(\bm{x}_i) - c\|_{\Sigma^{-1}}^2 \leq R^2 + \xi_i, \quad \xi_i \geq 0,\forall i,
%     \label{eq:objective}
% \end{align}
% Here we introduce a regularization term $\frac{1}{2} \|\Sigma\|_{\text{Fr}}^2$ as we don't want $\|\Sigma\|$ go to infinity. If $\Sigma = I$, then the optimization problem is identical to SVDD. After we find the optimal $R$, $c$ and $\Sigma$, we can view a new sample $Y$ as out-of-domain data, if $\Phi(Y)$ isn't in the hyper-ellipsoid  $\|\Phi(\bm{x}) - c\|_{\Sigma^{-1}}^2 = R^2$.

% For computational simplicity, we use $\hat{\mu}$ and $\hat{\Sigma}$ to replace $c$ and $\Sigma$, where $\hat{\mu}$ and $\hat{\Sigma}$ are the empirical mean and the empirical covariance matrix, defined as following:
% \begin{align}
%     \hat{\mu} =  \frac{1}{n} \sum_{i=1}^n f(\bm{x}_i) \quad \hat{\Sigma} =  \frac{1}{n-1} \sum_{i=1}^n (f(\bm{x}_i) - \hat{\mu}) (f(\bm{x}_i) - \hat{\mu})^\top.
% \end{align}

% So the final optimization problem we consider is:
% \begin{align*}
%     \min_{R, \xi} R^2 + \frac{1}{\nu n} \sum_i \xi_i, \quad \text{s.t.}\quad \|f(\bm{x}_i) - \hat{\mu}\|_{\hat{\Sigma}^{-1}}^2 \leq R^2 + \xi_i, \quad \xi_i \geq 0,\forall i,
% \end{align*}
% which can be solved with the standard optimization methods. And we find the optimal $R$, we can determine a new sample $Y$ is in-distribution data or out-of-domain data, by finding if the feature of $Y$ is inside the hyper-ellipsoid  $\|f(Y) - \hat{\mu}\|_{\hat{\Sigma}^{-1}}^2 = R^2$ or not.

% \noindent\paragraph{Connection with Density Estimation}\quad\quad
% % \tongzheng{This part can be abbreviated? Re-organize later.} 
% % Our proposed method is closely related to the Mahalanobis distance and Gaussian density estimation. Mahalanobis distance can be used to measure the distance between the point $X$ and the distribution $P$. Assume the mean of $P$ is $\bm{c}$ and the covariance of $P$ is $\bm{\Sigma}$, the Mahalanobis distance is defined via:
% % \begin{align*}
% %     D_{M}(\bm{x}, P) = \sqrt{(\bm{x} - \bm{c})^\top \bm{\Sigma}^{-1} (\bm{x} - \bm{c})}.
% % \end{align*}
% % Notice that, the criterion we use is exactly the Mahalanobis distance. And Mahalanobis distance is also related to the density of the Gaussian distribution. 
% Note that, our proposed method is equivalent to density estimation, if we further assume the feature of the data follows the Gaussian distribution, i.e. $\Phi(\bm{x})\sim\mathcal{N}(\bm{c}, \bm{\Sigma})$, where $c$ and $\bm{\Sigma}$ are the mean and the covariance of the Gaussian distribution. Under this assumption, the log-density function of $\Phi(\bm{x})$ can be written as:
% \begin{align*}
%     \log p(\Phi(\bm{x})) = &-\frac{1}{2} (\Phi(\bm{x})-\bm{c})^\top \bm{\Sigma}^{-1}(\Phi(\bm{x}) - \bm{c}) + \log Z \\
%     = &-\frac{1}{2}\|\Phi(\bm{x}) - \bm{c}\|_{\bm{\Sigma}^{-1}}^2 + \log Z\, .
% \end{align*}
% where $Z$ is the normalization constant (a.k.a the partition function) that is independent of $\Phi(\bm{x})$. Moreover, our approximation on decomposing the feature space into several subspace is in fact introducing an additional assumption that the feature from each layer is approximately independent:
% \begin{align*}
%     p(\Phi(\bm{x})) \approx \prod_{\ell=1}^L p(f_{\ell}\circ f_{\ell-1}\cdots \circ f_{1}(\bm{x}))\,.
% \end{align*}
% And then we have
% \begin{align*}
%     \log p(\Phi(\bm{x})) \approx & \sum_{l=1}^L \log p(f_{l}\circ f_{l-1}\cdots \circ f_{1}(\bm{x}))\\
%     % = & -\frac{1}{2}\sum_{l=1}^L (f_{l}\circ f_{l-1}\cdots \circ f_{1}(\bm{x}) - \bm{c}_l)^\top \bm{\Sigma}_{l}^{-1}(f_{l}\circ f_{l-1}\cdots \circ f_{1}(\bm{x}) - \bm{c}_l) + \log Z.
%     = & -\frac{1}{2}\sum_{\ell=1}^L \|f_{\ell}\circ f_{\ell-1}\circ\cdots \circ f_{1}(\bm{x}) - \bm{c}_\ell\|_{\bm{\Sigma}_\ell^{-1}}^2  \\
%     & + \log Z \, .
% \end{align*}
% Intuitively our method can be viewed as first estimating the density of the data $\bm{x}$, 
% by assuming the feature of the data $\Phi(\bm{x})$ follows a (layer-wise factorized) Gaussian distribution, 
% and then view the data with likelihood smaller than the threshold as the out-of-domain data. 
% This criterion has been widely used in the density estimation based out-of-domain detection \cite{nalisnick2018do,ren2019likelihood}, but generally
% the models they use are more complex than the Gaussian distribution.
